An analysis of incorporating an external language model into a sequence-to-sequence model

Attention-based sequence-to-sequence models for automatic speech recognition jointly train an acoustic model, language model, and alignment mechanism. Thus, the language model component is only trained on transcribed audio-text pairs. This leads to the use of shallow fusion with an external language model at inference time. Shallow fusion refers to log-linear interpolation with a separately trained language model at each step of the beam search. In this work, we investigate the behavior of shallow fusion across a range of conditions: different types of language models, different decoding units, and different tasks. On Google Voice Search, we demonstrate that the use of shallow fusion with a neural LM with wordpieces yields a 9.1% relative word error rate reduction (WERR) over our competitive attention-based sequence-to-sequence model, obviating the need for second-pass rescoring.

==> X.tex <==
\relax 
\citation{Chan15}
\citation{Bahdanau16}
\citation{Graves12}
\citation{Graves06}
\citation{RohitSeq17}
\citation{RohitSeq17}
\citation{Rafal16}
\citation{Chan15}
\citation{Bahdanau16}
\citation{Gulcehre15}
\citation{Jan17}
\citation{Gulcehre15}
\citation{Hori17}
\citation{ColdFusion17}
\citation{Gulcehre15}
\citation{Jan17}
\providecommand \oddpage@label [2]{}
\newlabel{SEC:INTRODUCTION}{{1}{1}}
\@writefile{toc}{\contentsline {section}{\numberline {1} Introduction }{1}}
\@writefile{toc}{\contentsline {section}{\numberline {2} Shallow fusion with LAS models}{1}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1} Listen, attend, and spell}{1}}
\citation{HochreiterSchmidhuber97}
\citation{Tu16}
\citation{Jan17}
\citation{Yonghui16}
\citation{Chan15}
\citation{wordpiece_schuster}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces The dotted line box shows the basic LAS model, including an encoder, attention, and decoder. In shallow fusion, an external LM is incorporated via log-linear interpolation.\relax }}{2}}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:las_lm}{{1}{2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2} Integrating a language model}{2}}
\@writefile{toc}{\contentsline {section}{\numberline {3} Exploring shallow fusion across tasks, decoding units, and types of language models}{2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1} Tasks: WSJ vs. Google Voice Search}{2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2} Decoding Units: Wordpieces vs. Graphemes}{2}}
\citation{Jan17}
\citation{Bahdanau16}
\citation{Gulcehre15}
\citation{Sennrich15}
\citation{Mikolov2010}
\citation{Bahdanau16}
\citation{Mohri2002}
\citation{Allauzen2007}
\citation{Allauzen2011}
\citation{Rafal16}
\citation{Jan17}
\citation{Schuster97}
\citation{Jan17}
\citation{Povey2011}
\citation{Vaswani17}
\citation{Hasim15}
\citation{Golan16}
\citation{AbadiAgarwalBarhamEtAl15}
\citation{Allauzen2011}
\citation{Rao17}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3} Language Models: RNNs vs. $n$-gram}{3}}
\newlabel{SEC:EXPERIMENTS}{{4}{3}}
\@writefile{toc}{\contentsline {section}{\numberline {4} Experimental details }{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1} Wall Street Journal}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2} Google Voice Search}{3}}
\bibstyle{IEEEbib}
\bibdata{main}
\bibcite{Chan15}{1}
\newlabel{SEC:RESULTS}{{5}{4}}
\@writefile{toc}{\contentsline {section}{\numberline {5} Results }{4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1} Comparing LMs for shallow fusion}{4}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces WER of \textsc  {las-g} fused with various LMs. While word constraints do help the $n$-gram LM, \textsc  {rnn-g} performs even better.\relax }}{4}}
\newlabel{table:wsj_char}{{1}{4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2} Extending shallow fusion to wordpiece models}{4}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces WER of \textsc  {las-wp} combined with various LMs on WSJ. \textsc  {rnn-wp} again performs best.\relax }}{4}}
\newlabel{table:wsj_wpm}{{2}{4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3} Scaling up to Voice Search}{4}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces WER of shallow fusion of LAS with production $n$-gram LMs and an RNN LM. The RNN LM captures all the benefits of \textsc  {prodlm2} in a compact form. \relax }}{4}}
\newlabel{table:vs_lm}{{3}{4}}
\newlabel{SEC:CONCLUSIONS}{{6}{4}}
\@writefile{toc}{\contentsline {section}{\numberline {6} Conclusions }{4}}
\@writefile{toc}{\contentsline {section}{\numberline {7} Acknowledgements}{4}}
\bibcite{Bahdanau16}{2}
\bibcite{Graves12}{3}
\bibcite{Graves06}{4}
\bibcite{RohitSeq17}{5}
\bibcite{Rafal16}{6}
\bibcite{Gulcehre15}{7}
\bibcite{Jan17}{8}
\bibcite{Hori17}{9}
\bibcite{ColdFusion17}{10}
\bibcite{HochreiterSchmidhuber97}{11}
\bibcite{Tu16}{12}
\bibcite{Yonghui16}{13}
\bibcite{wordpiece_schuster}{14}
\bibcite{Sennrich15}{15}
\bibcite{Mikolov2010}{16}
\bibcite{Mohri2002}{17}
\bibcite{Allauzen2007}{18}
\bibcite{Allauzen2011}{19}
\bibcite{Schuster97}{20}
\bibcite{Povey2011}{21}
\bibcite{Vaswani17}{22}
\bibcite{Hasim15}{23}
\bibcite{Golan16}{24}
\bibcite{AbadiAgarwalBarhamEtAl15}{25}
\bibcite{Rao17}{26}
\@writefile{toc}{\contentsline {section}{\numberline {8} References}{5}}

